Application-aware Energy Attack Mitigation in the Battery-less Internet of Things

We study how to mitigate the effects of energy attacks in the batteryless Internet of Things (IoT). Battery-less IoT devices live and die with ambient energy, as they use energy harvesting to power their operation. They are employed in a multitude of applications, including safety-critical ones such as biomedical implants. Due to scarce energy intakes and limited energy buffers, their executions become intermittent, alternating periods of active operation with periods of recharging their energy buffers. Experimental evidence exists that shows how controlling ambient energy allows an attacker to steer a device execution in unintended ways: energy provisioning effectively becomes an attack vector. We design, implement, and evaluate a mitigation system for energy attacks. By taking into account the specific application requirements and the output of an attack detection module, we tune task execution rates and optimize energy management. This ensures continued application execution in the event of an energy attack. When a device is under attack, our solution ensures the execution of 23.3% additional application cycles compared to the baselines we consider and increases task schedulability by at least 21%, while enabling a 34% higher peripheral availability.

==> model.tex <==

\section{System Model} \label{s:system} \label{sec:design}

\hrule
The proposed EAM framework, as shown in Fig. \ref{f:ea}, consists of \emph{application manager}, \emph{task scheduler/ peripheral control}, and \emph{energy management} modules. An \emph{energy attack}, as shown in Fig. \ref{f:ea}, is characterized by $V_a(t)$. It is an event that asserts control on the ambient energy ($V_n(t), I_n(t)$) supplied to the intermittent computing device. The energy attack parameters are provided in an information set, $\mathbf{A}$, by the attack detection block that detects the occurrence of the attack using support vector machines ~\cite{mottola2023energy}. 
 The application manager selects the application profile (like normal, low-power, critical, short or long attack) and corresponding task rates based on application specifications. These tasks are then scheduled and correspondingly the peripherals are controlled in the intermittent computing device. The energy management unit controls the federated energy harvesting that considers the upcoming sequence of tasks while dynamically charging the federated capacitors. Overall, the framework efficiently manages the application execution during the energy attack by selecting the attack profile and the required tasks (execution supported by the federated energy harvesting buffers) in order to meet the application (task-rate) requirements.
EAM increases the schedulability of the application-tasks by at least 20\% and executes at least 10 more application cycles per hour. Additionaly, it also ensures an increased (at least 34.02\% higher) and an earlier (at least by 14 s) availability of the device peripherals as compared to the state-of-the-art.


\begin{figure}[!htb]
\centering
\vspace{-0.15in}
\includegraphics[width=3.5in]{Figure/system_ea.pdf}
\caption{Energy attack mitigation (EAM) in intermittent computing system.}
\vspace{-0.2cm}
\label{f:ea}
\end{figure}

\hrule

The application support in an intermittent computing predominantly depends on the ambient energy source availability. An attack on the energy source will impact the continued application support or the device requirements. 
The existing intermittent computing framework and the state-of-the-art federated harvesting and task scheduling schemes cannot mitigate an energy attack. Hence, we propose an energy attack mitigation (EAM) framework for intermittent computing system. It is illustrated in Fig.~\ref{f:arch}. We extend the concept of federated energy storage and use an application-aware energy manager that dynamically stores the harvested energy in isolated smaller capacitors. We consider $m$ energy buffers for storing the harvested energy from a source that could be under attack. 
\begin{figure}[htb]
\centering
\vspace{-0.15in}
\includegraphics[width=2.8in]{Figure/EAM_System_model_final.pdf}
\caption{EAM model details.}
\vspace{-0.2cm}
\label{f:arch}
\end{figure}
%\newtheorem*{Def1}{Definition 1}
%\begin{Def1}\label{def1}
%In a system with $\mathcal{T}$ types of UE ($i=1,\dots,T$), $s_i > s_j$ if $i<j$. 
%For example in a system with 3 types of users (i.e., ${\mathcal{T}}=3$), ${s}_3 > {s}_2 > s_1$.
%\end{Def1}
\begin{table}[!htp]
\caption{Energy attack Parameters in information set $\mathbf{A}$}
\small
\label{t:ea_param}
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 \bf{Parameter} & \bf{Symbol} \\ \hline
 Attack ongoing & $a_o$\\ \hline
 Attack ongoing accuracy & $a_{oa}$ \\ \hline
 Elapsed time & $a_{et}$  \\\hline
 Remaining time & $a_{rt}$\\  \hline
 \end{tabular}
\end{center}
\end{table}
The energy source attack detection module~\cite{mottola2023energy} monitors the energy attack information in the form of a set, $\mathbf{A}$, consisting of the parameters listed in Table \ref{t:ea_param}. This information set, $\mathbf{A}$, is sent to the {`\it{Energy management}'}, {`\it{Application Manager}'}, and {`\it{Task scheduler/ peripheral control}'} modules. These modules use the proposed `{\em{EAM Federated Harvesting (EAMFH) charging controller}}', `{\em{Profile selection and Application task manager}}', and `{\em{EAM task Scheduler and state assignment}}', respectively, to mitigate the energy attack. The application specification metrics, $\mathbf{M}$, provides a list of supported profiles and corresponding task rates required by the application. The energy attack detection information, $\mathbf{A}$, is available to these blocks that mitigate the attack by selecting the application profile and task states accordingly. 

\subsection{Application Manager}
The intermittent computing devices can be used in diverse application domains like (but not limited to): environmental sensing and monitoring, on-body sensing and wearables, and large scale infrastructure monitoring~\cite{Hester2017}. The implementation in such a wide-range of use-cases requires an application manager that can select the appropriate execution profile, $\rho$, task set, $\mathbf{T}$, and the task rates, $\mathbf{R}$. The application task set is managed by the application manager based on the profile $\rho$ selected.

The application specifications are provided by the developer in the form of metrics $\mathbf{M}$ that are listed in Table \ref{t:met}. The profiles that the application can support are based on the mode of system operation: under attack, low-power, or normal. The application-level task (ALT) set is predefined for a given application. The rate of these ALTs are specified for each of the supported profiles. The task dependency is also provided as a finish to start task list. Task based energy requirements are specified by a declarative software interface.
\begin{table}[!htp]
\small
\caption{Application specifications (metrics) $\mathbf{M}$}
\label{t:met}
\begin{center}
\begin{tabular}{|p{0.95in}|p{2.2in}|} 
 \hline
 \bf{Metric} & \bf{Significance} \\ \hline
{\bf \!\!\!Supported Profiles\!\!} & \!\!\!Short-attack (SA), long-attack (LA), normal (NML), low power (LP), critical (CTL)\\ \hline
{\bf ALT set} & {\{Tasks\}}\\ \hline
{\bf Task rate} & {Profile: \{Tasks (Rate)\}}\\ \hline
{\bf Task dependency} & {\{Finish-to-start Task Lists\}}\\ \hline
%{\bf System-level task set} & Sense, store, process, send\\ \hline
\end{tabular}
\end{center}
\end{table}

The transition diagram for system profile state is shown in Fig. \ref{f:ex2}(a). The application manager selects the system profile based on the intermittent computing device energy $E$ and energy attack parameter $a_{rt}$. When the attack is ongoing (i.e. $a_o=1$), if the remaining time of the attack is greater than the threshold time$\alpha$, i.e. $a_{rt}\geq \alpha$, then the LA, else SA profile is selected. The energy level thresholds $\Omega_0$ and $\Omega_1$, $\Omega_1>\Omega_0$, are used to select between the NML, LP, and CTL profiles. When the attack is not ongoing (i.e. $a_o=0$), if $E>\Omega_1$ then NML, else if  $E<\Omega_0$ then CTL, else LP profile is selected. The system state (energy level and energy attack information) is updated periodically and the profile selection is based on the current state of the system.
\begin{figure}[htb]
\centering
\includegraphics[width=3.5in]{Figure/Mode_transitions.pdf}
\vspace{-0.25cm}
\caption{Transition Diagrams for: (a) System Profile (b) Task State}
\vspace{-0.2cm}
\label{f:ex2}
\end{figure}

The steps of the proposed Profile Select and Application Task Manager module are given in Algorithm \ref{eamfh}, function I.
\subsection{Task Scheduler and Peripheral Control}
 The peripherals and resources that need energy in an intermittent computing system are: MCU (computing), sensors (sensing), and decision-control unit (actuator control)~\cite{Sahoo2021}. Each application task can be one of the four states shown in Fig. \ref{f:ex2}(b). Active tasks are set to be in ready state and the one being executed is in running state. Task dependency governs the task state. For example, a task is set to be in blocked state if it depends on another task that is yet to be executed. 

The information regarding the tasks is sent to the task Scheduler in the form of a set $\mathbf{T}$. The tasks are indexed as $\tau\in \mathbb{N}$ in accordance with the execution order that is governed by the task dependency specification of the application. The task scheduler sets the state of the tasks and controls the peripherals accordingly. It schedules tasks and selects task $\tau(n)$ for run-time execution during slot $n$. We set task state based on execution order and energy availability in buffers. We have used two small isolated capacitors for the federated energy storage. The energy stored in first capacitor is used for MCU and sensing. The energy stored in second capacitor is  used for decision-control unit. The transition of a `ready' to `running' state, for a task $\tau$, is performed when the energy available in the corresponding energy buffer ($E_{\mathcal{B}(\tau)}$) is greater than that required to execute the task ($\varepsilon(\tau)$). The power to the peripherals is controlled by mode selection (execution or sleep) based on the task scheduler.

The steps of the proposed EAM task scheduler module are given in Algorithm \ref{eamfh}, function II.

 
\subsection{Energy manager}
We consider an array of capacitors for federating the energy storage~\cite{Hester2015}. The lightweight tasks are performed using smaller capacitors that charge more quickly, whereas more power-intensive tasks can be performed using the energy stored in larger capacitors. Such a system consists of energy harvester and charging controller. The MCU turns on based on the energy harvesting output and the first stage capacitor voltage. The capacitors in the array are charged by the charging controller that requires the MCU to be turned on initially. The MCU initiates the proportional charging of the isolated federated energy buffers (small capacitors). 

The voltage equations of the energy harvesting circuit are obtained by assuming power from the energy source as $P(t)$ at time $t$. We consider a parallel resistor-capacitor circuit with the equivalent storage capacitor, $C_i$ in parallel to the resistor equivalent with the rest of the circuit's equivalent resistor, $R_p$. Hence the voltage of the capacitor, $C_i$ at time instance $t$ is given as:
\begin{equation}
    V_i(t)=\sqrt{P(t)\cdot R_p - e^\frac{-2t}{C_i\cdot R_p}\cdot \left( P\cdot R_p - V_0^2\right)}
\end{equation}
where $V_0$ is the capacitor voltage at $t=0$.

The energy harvesting power observed during slot $n$ from source to buffer $i$ is $P_i(n)$, which is governed by the proposed EAMFH control. The energy level in buffer $i$ at the beginning of slot $n$ is $E_i(n)$. %The energy budget of slot $n$ is $E(n)$. 
The energy level in buffer $i$ at the beginning of the next time slot is given as:
\begin{equation}
    E_i(n+1)=(1-\sigma_i)\cdot E_i(n)+\eta_i\cdot P_i(n)\cdot t %- \sigma_i\cdot E(n)
\end{equation}
where, the duration of a slot $n$ is $t$, the proportion of energy budget sourced by buffer $i$ is $\sigma_i$, and the efficiency of the energy buffer $i$ is $\eta_i$.
The energy management module dynamically charges the capacitors in order to sustain support of the active task at the earliest. 

The energy buffer, $\mathcal{B}(\tau)\in \mathbb{N}$, $\mathcal{B}(\tau)\leq m$ supports execution of task $\tau$. The EAM federated harvesting function proportionally stores the harvested energy in isolated buffers (small capacitors) based on the state of the task it supports. If the task $\tau$ is `ready' then a higher proportion of energy, $\Lambda_\tau$ is stored in the corresponding buffer, else a lower proportion of energy, $\lambda_\tau$, is stored.
The steps of the proposed EAMFH control module are given in Algorithm \ref{eamfh}, function III.

% \subsection{Application Specifications, Task Classification, and KPI}

\section{Energy attack mitigation}
The energy attack mitigation algorithm, EAM, Algorithm \ref{eamfh}, comprises of three functions: \emph{profile\_select\_App\_Task\_Manager},  \emph{EAM\_} \emph{task\_scheduler}, and \emph{EAM\_federated\_harvesting}. Each of these functions implements the {\emph{`Application manager'}}, {\emph{`Task scheduler and peripheral control'}}, and {\emph{`Energy manager'}} modules described in Section \ref{s:system}, respectively.



\begin{algorithm}[!htb]
\small
\caption{ EAM: Energy-attack Mitigation}
\label{eamfh}
\begin{algorithmic}
\State \textbf{Input:} $\mathbf{A}$, $\mathbf{M}$\\
 \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{\!\!}
  \SetKwFunction{FSub}{\!\!}
% Write Function with word ``Function''
  \SetKwProg{Fn}{Function I: Profile\_Select\_App\_Task\_Manager}{:}{}
  \Fn{\FSum{$\mathbf{A}$,$\mathbf{M}$}}{
        % a = first
        % b = second
        % sum = first + second
        % \KwRet sum
\begin{enumerate}
 \item {\bf Select profile $\rho$:} 
  \end{enumerate}
  ${}$\hspace{1.1em}{\bf if} $a_o=1$ and $a_{oa}>a_{oa}^{th}$ \\
  ${}$\hspace{2.5em}{\bf if} $a_{rt}>\alpha$ \\
   ${}$\hspace{3.25em}$\rho=1$, i.e. LA\\
   ${}$\hspace{2.5em}{\bf else} \\
   ${}$\hspace{3.25em}$\rho=2$, i.e. SA\\
   ${}$\hspace{2.5em}{\bf end if} \\
   ${}$\hspace{1.1em}{\bf else }  \\
  ${}$\hspace{2.5em}{\bf if} $\omega_o<E\leq \omega_1$  \\
   ${}$\hspace{3.25em}$\rho=3$, i.e. LP\\
   ${}$\hspace{2.5em}{\bf else if} $E<\omega_0$ \\
   ${}$\hspace{3.25em}$\rho=4$, i.e. CTL\\
   ${}$\hspace{2.5em}{\bf else} \\
   ${}$\hspace{3.25em}$\rho=5$, i.e. NML\\
      ${}$\hspace{2.5em}{\bf end if} \\
   ${}$\hspace{1.1em}{\bf end if}  \\
  
\begin{enumerate}
\item [2)] {\bf Select task set:} \newline Include task $\tau$ in task set $\mathbf{T}$ if it is enabled for \newline profile $\rho$, i.e $\mathbf{M}(\tau,\rho)>0$
\end{enumerate}
  %${}$\hspace{1.0em}{\bf for each} $i=1$ to $N$ \\
 % ${}$\hspace{4.0em}
 % ${}$\hspace{1.0em}Assign user $i$ to cluster $k^\star$, $k^\star=\underset{k}{\min}\,\, d^2(u_i,c_k)$ \\
  \begin{enumerate}
\item [3)] {\bf Assign task rate:} $\mathbf{R}(\tau)=\mathbf{M}(\tau,\rho)$
\end{enumerate}
\KwRet $\rho$, $\mathbf{T}$, $\mathbf{R}$
}
\noindent\SetKwProg{Fn}{Function II: EAM\_task\_scheduler}{:}{}
  \Fn{\FSub{$\rho$, $\mathbf{T}$, $\mathbf{R}$, $\mathbf{A}$}}{
\begin{enumerate}
     \item [1)] {\bf Set task state (when there is no energy attack):}
\end{enumerate}
  ${}$\hspace{1.2em}{\bf for each task} $\tau\in \mathbf{T}$ \\
  ${}$\hspace{1.5em}{\bf if}\,($E_{\mathcal{B}(\tau)}\geq\varepsilon(\tau)$)\,and\,($\tau=1$\,or\,$\mathbf{S}(\tau-1)=$`running')\\
   ${}$\hspace{3em}{\bf set} $\mathbf{S}(\tau)=$`ready' \\
  ${}$\hspace{1.5em}{\bf else}  \\
   ${}$\hspace{3em}{\bf set} $\mathbf{S}(\tau)=$`blocked' \\
     ${}$\hspace{1.5em}{\bf end if}  \\
  
  \begin{enumerate}
     \item [2)] {\bf Defer/ execute task in event of energy attack, $a_o=1$:}
\end{enumerate}
  ${}$\hspace{0.2em}{\bf for each task} $\tau\in \mathbf{T}$ \\
  ${}$\hspace{2.5em}{\bf if} $a_{rt}>(1/R(\tau))$ and $E_{\mathcal{B}(\tau)}>\varepsilon(\tau)$ \\
   ${}$\hspace{3em}{\bf set} $\mathbf{S}(\tau)=$`ready' \\
  ${}$\hspace{2.5em}{\bf else}  \\
   ${}$\hspace{3em}{\bf set} $\mathbf{S}(\tau)=$`blocked' \\
     ${}$\hspace{2.5em}{\bf end if}  \\
   
%   ${}$\hspace{3.2em}\#users in $k$: $N_k$, \#requesting $\tau$ of $p$: $n_\tau^p$\\
%   %${}$\hspace{4.0em}Compute no. of users \\
%   ${}$\hspace{3.2em}$\sigma_\tau^p=\frac{n_\tau^p}{N_k} $\\
    \begin{enumerate}
     \item [3)] {\bf Execution task $\tau(n)$ from the task set $\mathbf{T}$:}
\end{enumerate}
  ${}$\hspace{0.2em}{\bf for each task} $\tau\in \mathbf{T}$ \\
  ${}$\hspace{2.7em}{\bf if} $\mathbf{S}(\tau)=$`ready' and $E_{\mathcal{B}(\tau)}\geq\varepsilon(\tau)$\\
    ${}$\hspace{3.7em}{\bf Set} $\tau(n)=\tau$\\
  ${}$\hspace{3.7em}{\bf Set} $\mathbf{S}(\tau)=$`running'\\
  ${}$\hspace{3.7em}{\bf Remove} $\tau$ from $\mathbf{T}$\\
    ${}$\hspace{2.7em}{\bf end if}  \\
%   ${}$\hspace{3.2em}$\textbf{I2MB(}\boldsymbol{\mathcal{D}}_{\textbf{min}}\!\textbf{)}$:$\overline\gamma\!\!=$least SINR, user subset\\ %requesting $\tau$ of $p$\\
%   ${}$\hspace{3.2em}$\textbf{I2MB(}\boldsymbol{\mathcal{C}\!r}_{\textbf{min}}\!\textbf{)}$:$\overline\gamma\!\!=$least SINR, all users set\\% requesting $\tau$ of $p$\\
%   ${}$\hspace{3.2em}Select $m_\tau^p=\min\limits_{m}(S\!I\!N\!R_{thr}(m)\geq\overline\gamma$)\\
  %\KwRet $q_\tau^p$
  \KwRet $\mathbf{S}$, $\tau(n)$
  }
\noindent\SetKwProg{Fn}{Function III: EAM\_federated\_harvesting}{:}{}
  \Fn{\FSub{$\rho$, $\mathbf{T}$, $\mathbf{R}$, $\mathbf{S}$}}{
  \begin{enumerate}
     \item [1)] {\bf Proportion of harvested energy to buffers}
\end{enumerate}
  ${}$\hspace{2em}{\bf for each buffer $i$} $=1$ to $m$\\
  ${}$\hspace{2.5em}{\bf for each $\tau \in$} $\mathbf{T}$\\
  ${}$\hspace{3em}{\bf if} $\mathbf{S}(\tau)=$`ready' or `running'\\
    ${}$\hspace{3.7em}{\bf Set} $P_{\mathcal{B}(\tau)}(n)=\Lambda_\tau\cdot P$\\
  ${}$\hspace{3em}{\bf else} \\
    ${}$\hspace{3.7em}{\bf Set} $P_{\mathcal{B}(\tau)}(n)=\lambda_\tau\cdot P$\\
      ${}$\hspace{3em}{\bf end if} \\
  \KwRet $\mathbf{P}$
  }

\noindent\textbf{Output:} $P_i(n)$
\end{algorithmic}
\end{algorithm}
\vspace{-0.1in}
\section{Example Applications}
\begin{figure}[htb]
\centering
\vspace{-0.15in}
\includegraphics[width=3.5in]{Figure/Examples_new.pdf}
\vspace{-0.2cm}
\caption{Application-level Tasks in example applications: (a) HVAC system (b) Greenhouse irrigation system (c) Controlled room ventilation system}
\vspace{-0.2cm}
\label{f:ex1}
\end{figure}
We consider three example applications: HVAC, greenhouse irrigation, and controlled room ventilation system. 
%\subsection{Application-level Task (ALT): Data Dependency and Profile-based Set}
The data dependency between ALTs for the considered applications is shown in Fig. \ref{f:ex1}.
\subsubsection{HVAC system (cf. Fig. \ref{f:ex1}(a))}
The temperature and humidity sensing task needs to be performed within every 15 min, respectively. This is followed by the decision task that sends the decision to the actuator control. Hence, the actuator control is performed once every 15 min and is essential before the next decision.
\subsubsection{Greenhouse irrigation system (cf. Fig. \ref{f:ex1}(b))}
The humidity sensing task is performed within every [5,30] min time window. This is followed by the decision task, which governs the sprinkler control. The sprinkler control is performed at least once every 30 min based on the decision. 
\subsubsection{Controlled room ventilation system (cf. Fig. \ref{f:ex1}(c))}
The temperature and CO$_2$ sensing task is performed within every 10 min. The decision task subsequently controls the ventilation through the window control task, both being performed at least once every 10 min. 

The corresponding ALT set and task dependency lists are given in Table \ref{t:alt}. The profile based ALT rates for the three applications are listed in Table \ref{t:rate}.



\begin{table}[!htp]
\small
\caption{ALT Set and Dependency}
\vspace{-0.1in}
\begin{center}
\begin{tabular}{|p{0.75in}|p{1.in}|p{1.3in}|} 
 \hline
 \bf{Application} & \bf{ALT set} & \bf{Task Dependency}\\ \hline
 {\bf HVAC}&\!\!\{TS, HS, D, AC\} & \{D(HS or TS), AC(D)\}\\ \hline
 %& Short-attack (SA), long-attack (LA), low power (LP), critical (CTL), normal (NML)\\ \hline
{\bf Greenhouse irrigation}&\{HS, D, SC\} & \{D(HS), SC(D)\}\\ \hline
    {\bf Room ventilation\!\!}&\!\!\{TS, CS, D, WC\}&\{D(TS or CS), WC(D)\}\\ \hline
%{\bf System-level task set} & Sense, store, process, send\\ \hline
\end{tabular}
\end{center}
HS: Humidity sensing, TS: Temperature sensing, CS: CO$_2$ sensing, AC: Actuator control, SC: Sprinkler control, WC: Window control, D: Decision
\label{t:alt}
\end{table}
\vspace{-0.1in}
\begin{table}[!htp]
\small
\caption{Profile based ALT}
\vspace{-0.1in}
\label{t:rate}
\begin{center}
\begin{tabular}{|p{0.55in}|p{0.25in}|p{0.25in}|p{0.25in}|p{0.25in}|p{0.25in}|p{0.25in}|} 
 \hline
 \bf{Application} & \bf{ALT}&\multicolumn{5}{c|}{\bf{Rate (per hour) based on Profile}} \\ \cline{3-7}
 &  & \bf{SA}&\bf{LA}&\bf{LP}&\bf{CTL}&\bf{NML}\\ \hline
 \multirow{5}{0.55in}{\bf HVAC}& TS& 8 &4 &12 &4 &30 \\ \cline{2-7}
& HS &8 &4 &12 &4 &30  \\ \cline{2-7}
& D&8 &4 &12 &4 &30 \\ \cline{2-7}
& AC&8 &4 &12 &4 &30\\ 
 \hline
  \multirow{4}{0.55in}{\bf Greenhouse irrigation}& HS&4 &2 &6 &2 &12\\ \cline{2-7}
& D&4 & 2& 6& 2&12 \\ \cline{2-7}
& SC&4 &2 &6 &2 &12\\ 
 \hline
  \multirow{5}{0.55in}{\bf Room ventilation}& CS& 20 &6 &15 &6 &45 \\ \cline{2-7}
& TS & 20 &6 &15 &6 &45 \\ \cline{2-7}
& D& 20 &6 &15 &6 &45  \\ \cline{2-7}
& WC& 20 &6 &15 &6 &45\\ 
 \hline
\end{tabular}
\end{center}
\end{table}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:
